Survey on AI-Generated Media Detection: From Non-MLLM to MLLM

The proliferation of AI-generated media poses significant challenges to information authenticity and social trust, making reliable detection methods highly demanded. Methods for detecting AI-generated media have evolved rapidly, paralleling the advancement of Multimodal Large Language Models (MLLMs). Current detection approaches can be categorized into two main groups: Non-MLLM-based and MLLM-based methods. The former employs high-precision, domain-specific detectors powered by deep learning techniques, while the latter utilizes general-purpose detectors based on MLLMs that integrate authenticity verification, explainability, and localization capabilities. Despite significant progress in this field, there remains a gap in literature regarding a comprehensive survey that examines the transition from domain-specific to general-purpose detection methods. This paper addresses this gap by providing a systematic review of both approaches, analyzing them from single-modal and multi-modal perspectives. We present a detailed comparative analysis of these categories, examining their methodological similarities and differences. Through this analysis, we explore potential hybrid approaches and identify key challenges in forgery detection, providing direction for future research. Additionally, as MLLMs become increasingly prevalent in detection tasks, ethical and security considerations have emerged as critical global concerns. We examine the regulatory landscape surrounding Generative AI (GenAI) across various jurisdictions, offering valuable insights for researchers and practitioners in this field.

==> Taxonomy/tax-mllm.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=8em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\large,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[!th]
    \centering
    \resizebox{0.96\textwidth}{!}{
                \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=5em,font=\large,}{},
            where level=2{text width=8em,font=\large,}{},
            where level=3{text width=8.8em,font=\large,}{},
            where level=4{text width=8em,font=\large,}{},
                [                
                    MLLM Detector
                    [
                        \hspace{0.5cm}Text
                         [
                           \hspace{0.4cm}Authenticity
                           [
                                \hspace{0.1cm}Statistical-based
                                [
                                HowkGPT~\cite{vasilatos2023howkgpt}{, }DNA-GPT~\cite{yang2023dna}{, }DetectLLM~\cite{su2023detectllm}{, }\\DetectGPT~\cite{mitchell2023detectgpt}{, }Fast-DetectGPT~\cite{bao2023fast}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.1cm}Prompt Engineering
                                [
                                LOKI~\cite{ye2024loki}{, }Bhattacharjee et al.~\cite{bhattacharjee2024fighting}{, }zhang et al.~\cite{zhang2024detection}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.1cm}Self-consistency
                                [
                                DetectGPT-SC~\cite{wang2023detectgpt}{, }SimLLM~\cite{nguyen2024simllm}{, }Zhu et al.~\cite{zhu2023beat}{, }\\Raidar~\cite{mao2024raidar}{, }Rewritelearning~\cite{rewritelearning}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.3cm}Multi-Author
                                [
                                MIXSET~\cite{zhang2024llm}{, }LLM-DetectAIve~\cite{abassy2024llm}{, }Beemo~\cite{artemova2024beemo}{, }LLMDetect~\cite{cheng2024beyond}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.3cm}Watermarking-based
                                [
                                Kirchenbauer et al.~\cite{kirchenbauer2023watermark}{, }Kirchenbauer et al.~\cite{kirchenbauerreliability}{, }\\Christ et al.~\cite{christ2024undetectable}{, }Unigram-Watermark~\cite{zhaoprovable}{, }PersonaMark~\cite{zhang2024personamark}
                                , leaf, text width=34em
                                ]
                           ]
                        ]
                        [
                           \hspace{0.3cm}Explainability
                           [
                           Ji et al.~\cite{ji2024detecting}
                           , leaf, text width=44.5em
                          ]
                        ]
                        [
                           \hspace{0.3cm}Localization
                           [
                           LLMDetect~\cite{cheng2024beyond}{, }GigaCheck~\cite{tolstykh2024gigacheck}
                           , leaf, text width=44.5em
                          ]
                        ]
                    ]
                          [
                        \hspace{0.4cm}Image
                         [
                           \hspace{0.4cm}Authenticity
                           [
                                \hspace{0.1cm}Prompt Engineering
                                [
                                LOKI~\cite{ye2024loki}{, }Shield~\cite{shi2024shield}{, }Jia et al.~\cite{jia2024can}{, }VisuaCritic~\cite{huang2024visualcritic}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.3cm}Fine-tuning
                                [
                                $\textit{X}^2$-DFD~\cite{chen2024textit}{, }Fakeshield~\cite{xu2024fakeshield}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.1cm}External detectors
                                [
                                $\textit{X}^2$-DFD~\cite{chen2024textit}{, }FFAA~\cite{huang2024ffaa}
                                , leaf, text width=34em
                                ]
                           ]
                        ]
                        [
                           \hspace{0.3cm}Explainability
                           [
                           $\textit{X}^2$-DFD~\cite{chen2024textit}{, }FFAA~\cite{huang2024ffaa}{, }Fakshield~\cite{xu2024fakeshield}{, }Forgerysleuth~\cite{sun2024forgerysleuth}{, }SIDA~\cite{huang2024sida}{, }ForgeryTalker~\cite{lianlarge}
                           , leaf, text width=44.5em
                          ]
                        ]
                        [
                           \hspace{0.3cm}Localization
                           [
                                \hspace{0.1cm}Mask+Image-Text
                                [
                                Forgerygpt~\cite{li2024forgerygpt}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.1cm}Text+Image-Mask
                                [
                                Fakeshield~\cite{xu2024fakeshield}{, }SIDA~\cite{huang2024sida}{, }Editscout~\cite{nguyen2024editscout}
                                , leaf, text width=34em
                                ]
                           ][
                                \hspace{0.1cm}Independent Mask
                                [
                                ForgeryTalker~\cite{lianlarge}
                                , leaf, text width=34em
                                ]
                           ]
                        ]
                ] 
                          [
                           \hspace{0.4cm}Video
                            [
                           \hspace{0.4cm}Authenticity
                            [
                                \hspace{0cm}Frame-Level detector
                                [LOKI~\cite{ye2024loki}{, }MM-Det~\cite{song2024learning}{, }VANE-Bench~\cite{bharadwaj2024vane}
                                , leaf, text width=34em
                                ]
                            ]
                            [
                                \hspace{0cm}Watermarking-based
                                [
                                Li et al.~\cite{li2024video}
                                , leaf, text width=34em
                                ]
                            ]
                           ]
                            [
                           \hspace{0.3cm}Explainability
                                [
                           N/A
                           , leaf, text width=44.5em
                                ]
                            ]
                            [
                           \hspace{0.3cm}Localization
                                [
                                N/A
                                , leaf, text width=44.5em
                                ]
                            ]
                        ]
                        [
                           \hspace{0.4cm}Audio
                            [
                           \hspace{0.4cm}Authenticity
                            [
                                LOKI~\cite{ye2024loki}{, }SONICS~\cite{rahman2024sonics}
                                , leaf, text width=44.5em
                            ]
                           ]
                            [
                           \hspace{0.3cm}Explainability
                                [
                           N/A
                           , leaf, text width=44.5em
                                ]
                            ]
                            [
                           \hspace{0.3cm}Localization
                                [
                                N/A
                                , leaf, text width=44.5em
                                ]
                            ]
                        ]
                        [
                           \hspace{0cm}Multi-modal
                            [
                           \hspace{0.4cm}Authenticity
                                [
                                \hspace{0.4cm}Text-Image
                                [
                                SNIFFER~\cite{qi2024sniffer}{, }Cheap~\cite{wu2023cheap}
                                , leaf, text width=34.5em
                                ]
                                ]
                                [
                                \hspace{0.4cm}Visual-Audio
                                [
                                Shahzad et al.~\cite{shahzad2024good}{, }V²A-Mark~\cite{zhang2024v2a}
                                , leaf, text width=34.5em
                                ]
                                ]
                           ]
                            [
                           \hspace{0.3cm}Explainability
                                [
                           N/A
                           , leaf, text width=44.5em
                                ]
                            ]
                            [
                           \hspace{0.3cm}Localization
                                [
                                N/A
                                , leaf, text width=44.5em
                                ]
                            ]
                        ]
                    ]
                    
        \end{forest}
    }
    \caption{Taxonomy of MLLM detecting AI-generated media ranging from unimodal to multimodal}
    \label{tax_of_mllm_detector}
\end{figure*}

==> Taxonomy/tax-non-mllm.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=8em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=center,font=\large,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]

\begin{figure*}[!th]
    \centering
    \resizebox{0.96\textwidth}{!}{
                \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=center,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=5em,font=\large,}{},
            where level=2{text width=8em,font=\large,}{},
            where level=3{text width=8.8em,font=\large,}{},
            where level=4{text width=8em,font=\large,}{},
                    [   
                        \hspace{0.3cm}Non-MLLM\\Detector
                        [
                        \hspace{0.5cm}Text
                         [
                           \hspace{0.4cm}Authenticity
                           [
                                \hspace{0.1cm}Stylistic-based
                                [
                                DeTeCtive~\cite{guo2024detective}{, }Shah et al.~\cite{shah2023detecting}{, }Kumarage et al.~\cite{kumarage2023stylometric}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.1cm}Linguistics-based
                                [
                                Hamed et al.~\cite{hamed2023improving}{, }Gallé et al.~\cite{galle2021unsupervised}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                           \hspace{0cm}Watermarking-based
                            [
                           Yoo et al.~\cite{yoo2023robust}{, }DeepTextMark~\cite{munyer2024deeptextmark}{, }Yang et al.~\cite{yang2023watermarking}{, }\\AWT~\cite{abdelnabi2021adversarial}{, }REMARK-LLM~\cite{zhang2024remark}
                           , leaf, text width=34em
                            ]
                           ]
                        ]
                        [
                           \hspace{0.3cm}Explainability
                           [
                           GPTZero~\cite{gptzero}{, }Mitrovic et al.~\cite{mitrovic2023chatgpt}{, }Ji et al.~\cite{ji2024detecting}
                           , leaf, text width=44.5em
                          ]
                        ]
                        [
                           \hspace{0.3cm}Localization
                           [
                           Zhang et al.~\cite{zhang2024machine}{, }MFD~\cite{tao2024unveiling}
                           , leaf, text width=44.5em
                          ]
                        ]
                    ]
                          [
                           \hspace{0.4cm}Image
                         [
                           \hspace{0.4cm}Authenticity
                           [
                                \hspace{0.1cm}High-Level based
                                [
                                FHAD~\cite{wang2024generated}{, }Fraid~\cite{farid2022lighting,farid2022perspective}{, }Sarkar et al.~\cite{sarkar2024shadows}{, }AIDE~\cite{yan2024sanity}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.1cm}Low-Level based
                                [
                                PatchCraft~\cite{zhong2024patchcraft}{, }LGrad~\cite{tan2023learning}{, }AUSOME~\cite{poredi2023ausome}{, }\\Wolter et al.~\cite{wolter2022wavelet}{, }Synthbuster~\cite{bammey2023synthbuster}{, }Frank et al.~\cite{frank2020leveraging}{, }\\Corvi et al.~\cite{corvi2023intriguing}{, }SeDID~\cite{ma2023exposing}{, }E3~\cite{azizpour2024e3}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.1cm}Reconstruction \\Error based
                                [
                                DIRE~\cite{wang2023dire}{, }AEROBLADE~\cite{ricker2024aeroblade}{, }FIRE~\cite{chu2024fire}{, }\\DRCT~\cite{chendrct}{, }SemGIR~\cite{yu2024semgir}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                           \hspace{0cm}Watermarking-based
                            [
                           EditGuard~\cite{zhang2024editguard}{, }DiffusionShield~\cite{cui2023diffusionshield}{, }ZoDiac~\cite{zhang2024robust}{, }\\LaWa~\cite{rezaei2024lawa}{, }WMAdapter~\cite{ci2024wmadapter}
                           , leaf, text width=34em
                            ]
                           ]

                        
                        ]
                        [
                           \hspace{0.3cm}Explainability
                           [
                           Cifake~\cite{bird2024cifake}{, }ASAP~\cite{huang2024asap}
                           , leaf, text width=44.5em
                          ]
                        ]
                        [
                           \hspace{0.3cm}Localization
                           [
                           DA-HFNet~\cite{liu2024hfnet}{, }DiffForensics~\cite{yu2024diffforensics}{, }MoNFAP~\cite{miao2024mixture}{, }HiFi-Net++~\cite{guo2024language}{, }SAFIRE~\cite{kwon2024safire}
                           , leaf, text width=44.5em
                          ]
                          ]
                          ]
                          [
                           \hspace{0.4cm}Video
                            [
                           \hspace{0.4cm}Authenticity
                           [
                                \hspace{0.1cm}Frame-Level
                                [
                                Bohacek et al.~\cite{bohacek2024human}{, }AIGVDet~\cite{bai2024ai}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                                \hspace{0.1cm}Video-Level
                                [
                                DIVID~\cite{liu2024turns}{, }He et al.~\cite{he2024exposing}{, }yan et al.~\cite{yan2024generalizing}{, }DuB3D~\cite{ji2024distinguish}{, }\\Demamba~\cite{chen2024demamba}{, }Vahdati et al.~\cite{vahdati2024beyond}
                                , leaf, text width=34em
                                ]
                           ]
                           [
                           \hspace{0cm}Watermarking-based
                            [
                           DVMark~\cite{luo2023dvmark}{, }REVMark~\cite{zhang2023novel}
                           , leaf, text width=34em
                            ]
                           ]
                        ]
                        [
                           \hspace{0.3cm}Explainability
                           [
                           N/A
                           , leaf, text width=44.5em
                          ]
                        ]
                        [
                           \hspace{0.3cm}Localization
                           [
                           N/A
                           , leaf, text width=44.5em
                          ]
                        ]
                          ]
                          [
                           \hspace{0.4cm}Audio
                            [
                            \hspace{0.4cm}Authenticity
                            [
                           \hspace{0.4cm}Fingerprint
                            [
                               Salvi et al.~\cite{salvi2024listening}
                               , leaf, text width=34em
                            ]
                           ]
                           [
                           \hspace{0cm}Watermarking-based
                            [
                               DeAR~\cite{liu2023dear}{, }AudioSeal~\cite{roman2024proactive}{, }Wu et al.~\cite{wu2023adversarial}
                               , leaf, text width=34em
                            ]
                           ]
                            ]
                            [
                           \hspace{0.3cm}Explainability
                           [
                           SLIM~\cite{zhu2024slim}{, }SFAT-Net-3~\cite{cuccovillo2024audio}{, }Pascu et al.~\cite{pascu2024easy}
                           , leaf, text width=44.5em
                          ]
                        ]
                        [
                           \hspace{0.3cm}Localization
                           [
                           HarmoNet~\cite{liu2024harmonet}{, }CFPRF~\cite{wu2024coarse}
                           , leaf, text width=44.5em
                          ]
                        ]
                            ]
                          [
                           \hspace{0cm}Multimodal
                            [
                           \hspace{0.4cm}Authenticity
                                [
                                \hspace{0.4cm}Text-Image
                                [
                                HAMMER~\cite{Shao_2023_CVPR}
                                , leaf, text width=34.5em
                                ]
                                ]
                                [
                                \hspace{0.4cm}Visual-Audio
                                [
                                Li et al.~\cite{li2024zero}{, }Yoon et al.~\cite{yoon2024triple}
                                , leaf, text width=34.5em
                                ]
                                ]
                           ]
                            [
                           \hspace{0.3cm}Explainability
                                [
                           N/A
                           , leaf, text width=44.5em
                                ]
                            ]
                            [
                           \hspace{0.3cm}Localization
                                [
                                DiMoDif~\cite{koutlis2024dimodif}{, }MMMS-BA~\cite{katamneni2024contextual}
                                , leaf, text width=44.5em
                                ]
                            ]
                            ]
                          ]
                        ]

        \end{forest}
    }
    \caption{Taxonomy of Non-MLLM detecting AI-generated media ranging from unimodal to multimodal}
    \label{tax_of_non_mllm_detector}
\end{figure*}
